Decentralized dynamic task allocation for UAVs with limited communication range

We present the Limited-range Online Routing Problem (LORP), which involves a team of Unmanned Aerial Vehicles (UAVs) with limited communication range that must autonomously coordinate to service task requests. We first show a general approach to cast this dynamic problem as a sequence of decentralized task allocation problems. Then we present two solutions both based on modeling the allocation task as a Markov Random Field to subsequently assess decisions by means of the decentralized Max-Sum algorithm. Our first solution assumes independence between requests, whereas our second solution also considers the UAVs' workloads. A thorough empirical evaluation shows that our workload-based solution consistently outperforms current state-of-the-art methods in a wide range of scenarios, lowering the average service time up to 16%. In the best-case scenario there is no gap between our decentralized solution and centralized techniques. In the worst-case scenario we manage to reduce by 25% the gap between current decentralized and centralized techniques. Thus, our solution becomes the method of choice for our problem.

==> auctions.tex <==
%!TEX root = planes.tex

\section{Auction-based coordination}
\label{sec:auction-based}

One of the most common approaches to decentralized task allocation is to employ market-based mechanisms, and auctions in particular. As explained in~\cite{koenig2010progress}, the simplest auction-based mechanism for this scenario is that in which agents perform parallel, single-item auctions. The intuitive functioning of this mechanism is very simple: whenever there is some new information to consider (i.e.: ``a request has been fulfilled", or ``a new request has been submitted to the system"), the agents (re)auction all of the tasks. Thereafter, each plane bids for all tasks. Finally, the auctioneers assign each task to the bidder who has submitted the best bid.

This auction mechanism can not be directly employed in our scenario because of the communication range limitation. Firstly, because not all agents can bid for all requests. That is, a UAVs may not be in range of the auctioneer of a request, and hence can not bid for it. This can be easily overcome by allowing the planes to bid only on requests whose auctioneers are within range. However, notice that this limitation does affect the resulting allocations. As a consequence, the allocations computed using this mechanism are not necessarily optimal anymore. That is, the computed allocation $a_t$ may differ from $a_t^*$ above.

Secondly, there are no specific points in time where there is some new information to consider. Because the UAVs are constantly moving, their distance to each request is also constantly changing. Therefore, the allocation computed at time $t$ may be different than the allocation computed at $t+1$, even if no request has been fulfilled, nor any new request entered the system. Hence, in this scenario it makes sense to compute a new allocation as soon as possible.

\begin{figure}
\centering
\includegraphics[width=.8\linewidth]{img/scenario2}
\caption{Example scenario.}
\label{fig:problem-example2}
\end{figure}

\begin{algorithm}
\caption{independent\_auctions$(p)$}
\label{alg:indpendent_auctions}
\begin{algorithmic}[1]
\While{$\lnot end$}
	\For{$r \in p.R$} \Comment{Time t}
		\State announce\_auction($r$)
	\EndFor 
	\For{$msg \in received\_auctions()$} \Comment{Time t+1}
		\State $distance \gets d(p, msg.r)$
		\State $send\_bid(msg.sender, msg.r, distance)$
	\EndFor
	\For{$r \in p.R$} \Comment{Time t+2}
		\State $winner \gets winner\_determination(bids, r)$
		\If{$winner \neq p$}
			\State $p.R \gets p.R \setminus {r}$
			\State $send\_win(winner, r)$
		\EndIf
	\EndFor
	\For{$msg \in received\_wins() $} \Comment{Time t+3}
		\State $p.R \gets p.R \cup \{msg.r\}$
	\EndFor
\EndWhile
\end{algorithmic} 
\end{algorithm}

Algorithm~\ref{alg:indpendent_auctions} outlines the basic operations performed by every UAV $p$ employing this coordination mechanism. We will see how this procedure works by following an example. Figure~\ref{fig:problem-example2} presents the same situation of Figure~\ref{fig:problem-example}. In this case, we have removed the communication range circles removed for clarity. Also, the red solid line connecting a plane to a target mean that the plane is the \emph{owner} of that request at that point in time. Finally, all lines are labeled by the distance they represent. Back to algorithm~\ref{alg:indpendent_auctions}, we can now see what the planes would do in this scenario. First, in lines [2-4], the planes that own some request(s) announce new auctions for them. In our example, plane A announces an auction of request 2 by sending a broadcast message. Likewise, plane C does the same thing for request 2, and B does it for request 3. At the next step, the planes start by bidding to all auctions that they see. As expressed in line 6, their bid is precisely their distance to the request being auctioned. Because UAVs A and B are within range, B receives the auction opened by A for request 2. Hence, it replies that with a bid message of value 2. Likewise, A receives B's auction announcement for request 3, and bids with value 2. Also, every UAV receives its own auction announcements, and bids for those requests. That is, UAV A bids for request 2 with a value of 5, B bids for 1 with a value of 7, and C bids for 3 with value 1. Next, in line 10, the UAVs that opened some auction proceed to collect the bids for that auction and determine the auction's winner (the bid with lowest value). In our case, plane C is the winner of request 1, because it is the only bidder. The winner of request 2 is plane B. Because B is not the current owner of request 2, the request has to be transferred to the winner (lines 12-13). Analogously, C wins request 3, which is transferred to it. Finally, the planes collect any tasks that they have won during the latest allocation procedure. In our example, plane B now becomes the owner of request 2 and C the owner of request 3. At the end of each iteration of that algorithm, each UAV ends up knowing which requests have been allocated to itself ($p.R$). 

%\begin{itemize}
%\item There are $tasks(t)$ parallel auctions, where $tasks(t)$ stands for the number of tasks at time $t$
%\item Parallel auctions are jointly started every period of time $T$
%\item Each auction is run by a plane for a single task
%\item Each plane (auctioneer) auctions all its tasks in separate, independent auctions
%\item Each auction is a one-shot (single-round) reverse auction. Each auctioneer issues a request for bids. The planes within the communication range of the auctioneer can participate in the auction by submitting their bids.
%\item Bidding policy of each plane defined as follows:
%
%$$a b$$
%
%\item Once an auctioneer receives bids from the planes in its communication range, it clears the auction by choosing the bid with minimum value, which stands for the plane that is closest to the task at auction.
%
%\end{itemize}

==> notation.tex <==
%!TEX root = planes.tex

\section*{Notation}
\begin{itemize}
 \item $R = \{\tau_1,\ldots,\tau_m\}$:  set of requests
 \item $r$: index used for requests.
 \item $P = \{\rho_1,\ldots,\rho_n\}$: set of planes
 \item $p$: index used for planes.
 \item $R_p \subseteq R$: set of requests that plane $p$ can serve.
 \item $P_r \subseteq P$: set of planes that can serve request $r$.
 \item $x_r$: variable that takes values in $P_r$.  $x_r=\rho_p$ encodes that plane $\rho_p$ serves request $\tau_r$.
 %\item $x_i$: variable for request $r_i$.
 %\item $D_j$: possible values of $x_i$.
 \item $X=\{x_r \forall r \in R\}$ is the set of all variables (one per request)
 \item $\mathbf{x}_r \in P_r$ an assignment to variable $x_r$.
 \item $\mathbf{X}$: an assignment of values to each of the variables in $X$.
  \item $\mathbf{X}^*$: optimal assignment of values to each of the variables in $X$.
 %\item $p_j \in P$: UAV 
 \item $X_p \subseteq X$: the set of variables related to UAV $\rho_p$. 
 \item $\mathbf{X_p}$:  an assignment of values to each of the variables in $X_p$.
 \item $c_p$: Constraint evaluating the cost of servicing the requests assigned to plane $\rho_p$.
 \item $c_{pr}$: Constraint evaluating the cost of plane $\rho_p$ servicing request $\tau_r$.
 \item $|A|$: number of elements in set $A$.
 \item $|f|$ : number of elements in the domain of function $f$.
 
 \item $z_{pr}$ : binary variable. $z_{pr}$ is one if plane $\rho_p$ serves request $\tau_r$ and zero otherwise.
 \item $Z_r=\{z_{pr} p\in P_r\}$: set of variables encoding the assignment of request $\tau_r$.
 \item $\mu_{f\rightarrow z_{pr}}$ message sent from factor $f$ to variable $z_{pr}$.
 \item $\mu_{z_{pr}\rightarrow f}$ message sent from variable $z_{pr}$ to  factor $f$.
 \item $\mathbf{z}_{pr}$ an assignment to $z_{pr}.$
 \item $Z_f$: set of variable in the scope of $f$.
 \item $Z_{f_{-pr}}$  set of variable in the scope of $f$ excluding $z_{pr}$.
 \item $F_{pr}$ set of factors that have $z_{pr}$ in the scope.
 \item $F_{pr-f}$ set of factors that have $z_{pr}$ in the scope excluding factor $f$.
 \item $v_{pr}(z_{pr})$: if $z_{pr}= 1$ it returns the cost for plane $\rho_p$ of servicing request $\tau_r$ otherwise zero.
 \item $s_r(Z_r)$: selection factor for request $\tau_r$. It is a one and only one selection factor.     
\item $\nu_{f\rightarrow g} = \mu_{f\rightarrow g}(1) -  \mu_{f\rightarrow g}(0) $
 \item $Z_p\{z_{pr} r\in R_p\}$: set of variables encoding the assignment to UAV $\rho_p$.
 
 
 
 
\end{itemize}

